The Stability of Delaunay Triangulations

We introduce a parametrized notion of genericity for Delaunay triangulations which, in particular, implies that the Delaunay simplices of $\delta$-generic point sets are thick. Equipped with this notion, we study the stability of Delaunay triangulations under perturbations of the metric and of the vertex positions. We quantify the magnitude of the perturbations under which the Delaunay triangulation remains unchanged.

==> Makefile <==
#
# Makefile for stab I, IJCGA submission
# 20120730
#

TEXINPUTS := .:./styles//:

	export TEXINPUTS

papers=stab1 ijcga_stab1 inria_stab1 cgl_stab1

default: stab1.bbl

ijcga: ijcga_stab1.bbl

inria: inria_stab1.bbl

cgl: cgl_stab1.bbl

all: $(addsuffix .pdf,$(basename ${papers}))

bib: $(addsuffix .bbl,$(basename ${papers}))

%.pdf: %.tex $(wildcard *.tex)
	pdflatex $<
	pdflatex $<

%.bbl: %.pdf *.bib
	bibtex $(basename $<)
	pdflatex $(basename $<)
	pdflatex $(basename $<)

clean:
	rm -f *.bbl *.blg *.aux *.out *.log *.brf *.thm *.toc \
$(addsuffix .pdf,$(basename ${papers}))

cleanmax: clean
	rm -f *~ lablst.pdf


